A Bijection between Necklaces and Restricted Multisets

We present a proof of Swee Hong Chan's conjecture establishing a bijection between the set of necklaces of length $n$ with at most $q$ colors, and the set of periodic functions $f: \mathbb{Z}_{n}\to {0, 1, ..., q-1}$ whose weighted sum is divisible by $n$, where $q$ and $n$ are coprime positive integers.

==> future_work.tex <==
\section{Future Work}
In an article about power sums modulo a prime, Stanley and Odlyzko calculated the number of subsets $S$ of $\mathbb{Z}/n\mathbb{Z}$ satisfying $\sum_{x\in S}x^{m}=\alpha$ in $\mathbb{F}_{p}$\cite{MR493709}. Follow from this result, Li and Wan established several bounds for enumerating polynomial subset sums\cite{MR3857935}.
